Selectively Answering Visual Questions

Recently, large multi-modal models (LMMs) have emerged with the capacity to perform vision tasks such as captioning and visual question answering (VQA) with unprecedented accuracy. Applications such as helping the blind or visually impaired have a critical need for precise answers. It is specially important for models to be well calibrated and be able to quantify their uncertainty in order to selectively decide when to answer and when to abstain or ask for clarifications. We perform the first in-depth analysis of calibration methods and metrics for VQA with in-context learning LMMs. Studying VQA on two answerability benchmarks, we show that the likelihood score of visually grounded models is better calibrated than in their text-only counterparts for in-context learning, where sampling based methods are generally superior, but no clear winner arises. We propose Avg BLEU, a calibration score combining the benefits of both sampling and likelihood methods across modalities.

==> figures/errors.tex <==
\begin{figure}[h!] 
\begin{center}
\includegraphics[width=7cm]{figures/hallucination.jpeg}
\caption{Question \emph{``Alright see if you can see the ORCA serial number now.''}. The top 3 answers by PaLM2 Bison with their likelihood are ('31631036', -1.32), ('468563995', -1.41), ('4667926374', -1.41). They are neither in the image nor in the gold captions. The serial number is not in the image. Correctly, LLaVA 13B does not trigger a response in this case considering the question unanswerable.\label{fig:hallucination}}
\end{center}
\end{figure}

\begin{figure}[h!] 
\begin{center}
\includegraphics[width=7cm]{figures/missing_info.jpeg}
\caption{Question \emph{``What action is currently selected?''}. The top 3 answers by PaLM2 Bison with their likelihood are ('projects', -0.69), ('archives', -0.76), ('devices', -1.13). The correct answer is devices but this information is not in the gold captions, captions can never be complete. The captions are 'The computer digital monitor screen with some websites open to', 'A quick link bar has appeared on an Apple computer screen.', 'Computer menu bar with options: Devices, Repositories, Projects, Archives, and Documentation.', 'some type of MacBook or laptop device u CNA use', 'A VizWiz app that has an organizer and lists projects and archives.'. \label{fig:missing_info}}
\end{center}
\end{figure}

\begin{figure}[h!] 
\begin{center}
\includegraphics[width=7cm]{figures/useless.jpeg}
\caption{Question \emph{``Which one is the blue one?''}.The top 3 answers by PaLM2 Bison with their likelihood are ('blue', -0.47), ('second', -0.63), ('right', -0.82). The first answer is true but useless for a vision impared person. The top 3 answers by LLaVA 13B Bison are correct. They are ('right', -0.08), ('right', -0.08), ('right', -0.08).  person.\label{fig:useless}}
\end{center}
\end{figure}


==> figures/in_context_lu.tex <==
\begin{tabular}{l|rrrrr|rrrrr|rrrrr|rrrrr|}
 & \multicolumn{10}{c|}{\textbf{Large Multimodal Models (LMM)}} & \multicolumn{10}{c|}{\textbf{Large Language Models (LLM)}} \\
Model & \multicolumn{5}{c|}{\textbf{LLaVA 13B} (61.2\% acc @ 34.0\% trig)} & \multicolumn{5}{c|}{\textbf{Flamingo 3B} (20.5\% acc @ 71.7\% trig)} & \multicolumn{5}{c|}{\textbf{PaLM 2 Bison} (33.6\% acc @ 78.8\% trig)} & \multicolumn{5}{c|}{\textbf{Falcon} (18.5\% acc @ 87.0\% trig)} \\
Method & AUC & ECE$\downarrow$ & C@60 & C@70 & C@80 & AUC & ECE$\downarrow$ & C@60 & C@70 & C@80 & AUC & ECE$\downarrow$ & C@60 & C@70 & C@80 & AUC & ECE$\downarrow$ & C@60 & C@70 & C@80 \\
\midrule
\avgwbleu & 70.5 & 28.6 & 100.0 & 73.8 & 33.3 & 88.1 & 19.5 & 18.1 & 9.5 & 4.7 & 73.6 & 9.8 & 26.4 & 18.4 & 11.2 & 85.1 & 13.5 & 12.1 & 4.6 & 1.1\\
\midrule
Likelihood & 68.8 & 7.9* & 100.0 & 71.6 & 20.8* & 88.7 & 17.3 & 22.1 & 12.1 & 0.5 & 57.5* & 20.6* & 0.0* & 0.0* & 0.0* & 73.8* & 64.2* & 7.2 & 1.7 & 1.4\\
\midrule
Diversity & 70.4 & 6.8 & 100.0 & 67.2 & 8.7 & 77.6 & 12.4 & 11.4 & 7.2 & 3.7 & 75.0 & 39.9 & 10.1 & 10.1 & 10.1 & 86.2 & 31.3 & 11.8 & 0.0 & 0.0\\
Repetitions & 69.3 & 9.9 & 100.0 & 73.2 & 28.4 & 76.7 & 5.4 & 7.9 & 7.9 & 4.4 & 72.7 & 31.8 & 21.6 & 10.1 & 10.1 & 84.0 & 34.0 & 11.8 & 0.0 & 0.0 \\
\end{tabular}

\begin{table*}[t]
    \centering
    \footnotesize
    \resizebox{1.0\textwidth}{!}{%
    \input{figures/in_context_lu}
    }
    \caption{Calibration metrics on VizWiz-QA comparing LMMs on the left and LLMs (with gold image captions) on the right. Likelihood lags behind for LLMs but is comparable to \avgwbleu\ in LMMs. Large differences (10 points or more) between \avgwbleu and likelihood are marked with *. \avgwbleu{} performs above or comparable to alternative metrics. 
    Sampling repetition and diversity suffer from relying on exact match between answers.}
\end{table*}



